Automated Search for Configurations of Deep Neural Network Architectures

Deep Neural Networks (DNNs) are intensively used to solve a wide variety of complex problems. Although powerful, such systems require manual configuration and tuning. To this end, we view DNNs as configurable systems and propose an end-to-end framework that allows the configuration, evaluation and automated search for DNN architectures. Therefore, our contribution is threefold. First, we model the variability of DNN architectures with a Feature Model (FM) that generalizes over existing architectures. Each valid configuration of the FM corresponds to a valid DNN model that can be built and trained. Second, we implement, on top of Tensorflow, an automated procedure to deploy, train and evaluate the performance of a configured model. Third, we propose a method to search for configurations and demonstrate that it leads to good DNN models. We evaluate our method by applying it on image classification tasks (MNIST, CIFAR-10) and show that, with limited amount of computation and training, our method can identify high-performing architectures (with high accuracy). We also demonstrate that we outperform existing state-of-the-art architectures handcrafted by ML researchers. Our FM and framework have been released %and are publicly available to support replication and future research.

==> X-overview.tex <==
\section{Overview}
\label{sec:overview}

\subsection{Feature Models}

Feature modelling provides a compact representation of the products in a Software Product Line in terms of \emph{features} and \emph{relationships}. It aims to identify the differences and commonality among all these products. Features models can be used in various stages of a software development, from requirements definition \cite{VariantRequirements2001} to pieces of code\cite{FeatureOrientedProgramming2001}.

Cardinality-based feature models (CFM)\cite{CFM} is simple extension of FODA notation\cite{FODA}. It is a hierarchy of features where every feature has a feature cardinality by means of of an UML-like annotation. A feature cardinality is an interval of the form $[m..n]$ where 
\[ 
m \in N  \quad \textrm{and} \quad m \in N \cup \{*\}  \quad \textrm{and} \quad ( m<=n  \quad \textrm{or} \quad n=*)  
\]

 This extension allows to select multiple instances of the same feature type and include all its feature sub-trees.
 
 In addition to cardinality, we use the Extended Feature Model notation to take into account the attributes of the features, especially the leaf features.
 
 These improved representation have however few drawbacks, as they complicate the configuration semantics in comparison to FODA. The new constraints caused by this representation (cardinality interval gaps, dead cardinality, unbound cardinality) are not handled correctly by common constraints solvers such as CSP and SAT as they are not intended to handle infinite configuration space.
 Besides, these constraints solvers do not handle natively the large variety of attributes the Extended feature model includes.  
 
 In order to mitigate these obstacles, we will limit our study during the sampling and product generation steps to finite cardinality features. Besides we will implement during experimentation steps our features model attributes as "XOR" nodes to our feature.
 
 The semantics of a feature model we will be using are described in \ref{table:semantic_fm}.
 Our semantic is an extension the standard semantics with the concept of "instance" of a feature. The instances of $f_n$, are features of the same type $f_n$ denoted as $ f_n^k $
 
\begin{table}[h]
\begin{tabular}{ p{5cm} p{4cm} }

Semantic & Meaning \\
$ f_1 \Rightarrow f $ & \multicolumn{1}{p{3cm}}{$ f_1 $ is an optional  sub-feature of $f$ } \\
$ f_1 \Leftrightarrow  f $ & \multicolumn{1}{p{3cm}}{$f_1$ is a mandatory sub-feature of $f$}  \\
$ (f_1 \vee ... \vee f_n \Leftrightarrow  f) \wedge \bigcap_{i<j} \neg(f_i \vee f_j) $ & \multicolumn{1}{p{3cm}}{$f_1, ... f_n $ are alternative sub-features of $f$ }  \\
$ f_1 \vee ... \vee f_n \Leftrightarrow  f $ & \multicolumn{1}{p{3cm}}{$f_1, ... f_n $ are "or" sub-features of $f$ }  \\
$ \neg(f_1 \wedge  f_2) $ & \multicolumn{1}{p{3cm}}{$f_1$ excludes $f_2$}  \\
$ f_1 \Rightarrow f_2 $ & \multicolumn{1}{p{3cm}}{$f_1$ requires $f_2$}\\
$ f_n^k   $ & \multicolumn{1}{p{3cm}}{instance k of $f_n$} \\
$ f_1 \Rightarrow f_2(a_1,...,a_n)   $ & \multicolumn{1}{p{3cm}}{$f_1$ requires $f_2$ with the attributes of $f_2$ set to the values $\{a_1, ..., a_n\}$ }
\end{tabular}
\caption{Semantics of the extended feature model used in our implementation}
\label{table:semantic_fm}
\end{table}

This extended semantic requires a new set of constraints to support the cardinality and order of features:

\[  (f_i \Rightarrow f_n^k)  \Rightarrow  (\forall l < k: f_i \Rightarrow f_n^l)  \]

This means that any instance k of feature $f_n$ cannot be enabled unless all its previous instances $f_n^l$ with $l<k$ are enabled.

In the feature model presented in Figure \ref{fig:extended_feature_model}, the training feature requires a real attribute called TRAINING\_RATE. 
An other attribute of the feature "training" could be LOSS\_FUNCTION, which is a literal attribute and not a scalar. 
 
Besides, the feature "Architecture" contains one or more layers $L_i$ and each layer contains one or more neurons $n_i,_k$. 
 
\subsection{Artificial Neural Networks} 
In the field of Artificial Neural networks, every neuron can be described with its input signal and its output operation. The output operation of every neuron is described as follow 

\[ output = \sigma(\sum_{i} input_i * weight_i + bias) \]

where $\sigma$ is an activation function to be chosen for every layer.

This means that every neurons requires n+2 attributes, where n is the number of input it is connected to for neurons $n_i,_k , i>1$ and n is the size of the input vector for neurons $n_1,_k$
It we model a 2 fully-connected layers where every layer is made of 10 neurons and the input is 20 elements long, the amount of attributes to handle reaches 320.
This means that an exhaustive feature model would require a large amount of attributes to be described. Besides, recent architectures include not only fully connected layers, but a large variety of layers that have additional attributes and behave differently. Some of these layers are the Convolution Layers, Pooling Layers, the  

\subsubsection{Convolution Layers} 

Convolution layers are a set of pattern maps (feature maps in the jargon of Deep Neural Network) generated by convolving different filters with an input signal \cite{KrizhevskyCNN2012}. This allows to detect primitive attributes and reduces the number of weights and bias to be learned since the neurons of the same pattern share the same weights and bias.
These operation require additional attributes: The convolution kernel size, the stride (distance between receptive fields),  the depth (the number of features) and the padding.

\subsubsection{Pooling Layers}

Pooling layers don't have any learnable weights or bias. Their main role is to to retain some value of a neuron cluster. This value in most case is the average value of the cluster or its maximum value.
This allows to reduce the network complexity by keeping only one value for every cluster.
Pooling layers require the following attribute: kernel size, stride, padding and type of pooling (average, maximum). 

\subsubsection{Order of layers and branching}

The order of layers and the operations to be performed on the neurons are critical to the viability and the performance of a Deep Neural Network.
This constraints the features combination that can be found in final configurations. 
We should also be capable to model the branching and merging of layers that occur in some Deep Neural Network architectures.  

==> architectures/constraints_lenet5.tex <==
\begin{itemize}
    \item C78:not Architecture  or  Block1\_Cell1\_Input1\_Convolution
    \item C81:not Architecture  or  Block1\_Cell1\_Input2\_Zeros
    \item C82:not Architecture  or  Block1\_Cell1\_Operation1\_Void
    \item C83:not Architecture  or  Block1\_Cell1\_Operation2\_Void
    \item C84:not Architecture  or  Block1\_Cell1\_Combination\_Sum
    \item ....
    \item C124:not Architecture  or  not Block4\_Element2
    \item C125:not Architecture  or  not Block1\_Element3
    \item C137:not Architecture  or  not Block2\_Element3
    \item C138:not Architecture  or  not Block3\_Element2
    \item C139:not Architecture  or  not Block5
\end{itemize}

==> architectures/constraints_level5_original.tex <==
\begin{itemize}
    \item C78:not Architecture  or  Block1\_Cell1\_Input1\_Convolution
    \item C81:not Architecture  or  Block1\_Cell1\_Input2\_Zeros
    \item C82:not Architecture  or  Block1\_Cell1\_Operation1\_Void
    \item C83:not Architecture  or  Block1\_Cell1\_Operation2\_Void
    \item C84:not Architecture  or  Block1\_Cell1\_Combination\_Sum
    \item C85:not Architecture  or  Block1\_Cell1\_Output\_Cell
    \item C86:not Architecture  or  Block1\_Cell2\_Input1\_Pooling
    \item C89:not Architecture  or  Block1\_Cell2\_Input2\_Zeros
    \item C80:not Architecture  or  Block1\_Cell2\_Operation1\_Void
    \item C81:not Architecture  or  Block1\_Cell2\_Operation2\_Void
    \item C82:not Architecture  or  Block1\_Cell2\_Combination\_Sum
    \item C83:not Architecture  or  Block1\_Cell2\_Output\_Block 
    \item C84:not Architecture  or  Block2\_Cell1\_Input1\_Convolution
    \item C87:not Architecture  or  Block2\_Cell1\_Input2\_Zeros
    \item C88:not Architecture  or  Block2\_Cell1\_Operation1\_Void
    \item C89:not Architecture  or  Block2\_Cell1\_Operation2\_Void
    \item C100:not Architecture  or  Block2\_Cell1\_Combination\_Sum
    \item C101:not Architecture  or  Block2\_Cell1\_Output\_Cell
    \item C102:not Architecture  or  Block2\_Cell2\_Input1\_Pooling
    \item C105:not Architecture  or  Block2\_Cell2\_Input2\_Zeros
    \item C106:not Architecture  or  Block2\_Cell2\_Operation1\_Void
    \item C107:not Architecture  or  Block2\_Cell2\_Operation2\_Void
    \item C108:not Architecture  or  Block2\_Cell2\_Combination\_Sum
    \item C109:not Architecture  or  Block2\_Cell2\_Output\_Block 
    \item C110:not Architecture  or  Block3\_Cell1\_Input1\_Convolution
    \item C113:not Architecture  or  Block3\_Cell1\_Input2\_Zeros
    \item C114:not Architecture  or  Block3\_Cell1\_Operation1\_Void
    \item C115:not Architecture  or  Block3\_Cell1\_Operation2\_Void
    \item C116:not Architecture  or  Block3\_Cell1\_Combination\_Sum
    \item C117:not Architecture  or  Block3\_Cell1\_Output\_Block 
    \item C118:not Architecture  or  Block4\_Cell1\_Input1\_Dense\
    \item C119:not Architecture  or  Block4\_Cell1\_Input2\_Zeros
    \item C120:not Architecture  or  Block4\_Cell1\_Operation1\_Flatten
    \item C121:not Architecture  or  Block4\_Cell1\_Operation2\_Void
    \item C122:not Architecture  or  Block4\_Cell1\_Combination\_Sum
    \item C123:not Architecture  or  Block4\_Cell1\_Output\_Output
    \item C124:not Architecture  or  not Block4\_Element2
    \item C125:not Architecture  or  not Block1\_Element3
    \item C137:not Architecture  or  not Block2\_Element3
    \item C138:not Architecture  or  not Block3\_Element2
    \item C139:not Architecture  or  not Block5
    
\end{itemize}

==> architectures/full_lenet5.tex <==

\begin{multicols}{2}

    \begin{itemize}
      \item Input(input\_shape)
      \item Block 1
        \begin{itemize}
          \item Cell1
            \begin{itemize}
              \item Convolution(5x5, 1x1, 6, same,tanh)
              \item Void
              \item Zeros
              \item Void
              \item Sum
              \item Cell
            \end{itemize}
          \item Cell2
            \begin{itemize}
              \item Pooling(2x2, 1x1, average, valid)
              \item Void
              \item Zeros
              \item Void
              \item Sum
              \item Block(1)
            \end{itemize}
            
        \end{itemize}
      \item Block 2
        \begin{itemize}
          \item Cell1
            \begin{itemize}
              \item Convolution(5x5, 1x1, 16, same,tanh)
              \item Void
              \item Zeros
              \item Void
              \item Sum
              \item Cell
            \end{itemize}
          \item Cell2
            \begin{itemize}
              \item Pooling(2x2, 2x2, average, valid)
              \item Void
              \item Zeros
              \item Void
              \item Sum
              \item Block(1)
            \end{itemize}
        \end{itemize}
      \item Block 3
        \begin{itemize}
          \item Cell1
            \begin{itemize}
              \item Convolution(5x5, 1x1, 120, same,tanh)
              \item Flatten
              \item Zeros
              \item Void
              \item Sum
              \item Block(1)
            \end{itemize}
        \end{itemize}
      \item Block 4
        \begin{itemize}
          \item Cell1
            \begin{itemize}
              \item Dense(84, tanh)
              \item Void
              \item Zeros
              \item Void
              \item Sum
              \item Cell
            \end{itemize}
        \end{itemize}
    \end{itemize}
\end{multicols}

==> architectures/plain_lenet5.tex <==

\begin{itemize}
  \item Input(input\_shape)
  \item Block 1
    \begin{itemize}
      \item Cell1
        \begin{itemize}
          \item Convolution(5x5, 1x1, 6, same,tanh)
        \end{itemize}
      \item Cell2
        \begin{itemize}
          \item Pooling(2x2, 1x1, average, valid)
        \end{itemize}
      \item Cell3
        \begin{itemize}
          \item Convolution(5x5, 1x1, 16, same,tanh)
        \end{itemize}
      \item Cell4
        \begin{itemize}
          \item Pooling(2x2, 2x2, average, valid)
        \end{itemize}
      \item Cell5
        \begin{itemize}
          \item Convolution(5x5, 1x1, 120, same,tanh)
          \item Flatten
        \end{itemize}
      \item Cell6
        \begin{itemize}
          \item Dense(84, tanh)
        \end{itemize}
      \item Cell7
        \begin{itemize}
          \item Dense(nb\_output\_classes, softmax)
        \end{itemize}
    \end{itemize}
\end{itemize}

